Design of Policy-Aware Differentially Private Algorithms

The problem of designing error optimal differentially private algorithms is well studied. Recent work applying differential privacy to real world settings have used variants of differential privacy that appropriately modify the notion of neighboring databases. The problem of designing error optimal algorithms for such variants of differential privacy is open. In this paper, we show a novel transformational equivalence result that can turn the problem of query answering under differential privacy with a modified notion of neighbors to one of query answering under standard differential privacy, for a large class of neighbor definitions. We utilize the Blowfish privacy framework that generalizes differential privacy. Blowfish uses a {\em policy graph} to instantiate different notions of neighboring databases. We show that the error incurred when answering a workload $\mathbf{W}$ on a database $\mathbf{x}$ under a Blowfish policy graph $G$ is identical to the error required to answer a transformed workload $f_G(\mathbf{W})$ on database $g_G(\mathbf{x})$ under standard differential privacy, where $f_G$ and $g_G$ are linear transformations based on $G$. Using this result, we develop error efficient algorithms for releasing histograms and multidimensional range queries under different Blowfish policies. We believe the tools we develop will be useful for finding mechanisms to answer many other classes of queries with low error under other policy graphs.

==> 1dmarginals.tex <==
%!TEX root=paper.tex

In this section, we consider the problem of releasing one dimensional marginals over a $d$-dimensional dataset under $G^1_{k^d}$. We first briefly describe our strategy for releasing a histogram (marginal on a one-dimensional dataset). We then present our strategy for releasing marginals on a $d$-dimensional dataset using {\em policy graph marginalization}. 


\subsubsection{Histogram under $G^1_k$}
In one dimension, the marginal is just a histogram. Hence the workload is the identity matrix $\mathbf{I}$. We already saw (in \csec\ref{sec:range-1Dline}) that the transformed database $\mathbf{x}_G$ under the line graph is the set of prefix counts. The transformed workload $\mathbf{I}_G$ under the line graph is the difference between adjacent prefix counts; i.e. $\mathbf{x}_G[i] - \mathbf{x}_G[i-1]$. Thus, we could (a) obtain noisy counts $\tilde{\mathbf{x}}_G$ using the Laplace mechanism, and (b) compute the histogram on the original database as the difference of adjacent counts in $\tilde{\mathbf{x}}_G$. This strategy will incur $O(1/\epsilon^2)$ error per count -- no better than using Laplace mechanism on the original set of counts. This is because the transformed workload is no easier to answer under differential privacy than the original workload (in fact, $\mathbf{I}_G$ is harder than $\mathbf{I}$).

However, in this case, the counts in the transformed database $\mathbf{x}_G$ are non-decreasing. We can use this property of $\mathbf{x}_G$ to reduce error by enforcing the non-decreasing constraint on the noisy counts $\tilde{\mathbf{x}}_G$. Hay et al \cite{vldb:HayRMS10} present a simple algorithm to postprocess the counts so that the error depends on the number of distinct counts in $\mathbf{x}_G$. Note that whenever a count in $\mathbf{x}$ is $0$, a pair of consecutive prefix sums in $\mathbf{x}_G$ are the same. Therefore, the number of distinct values in $\mathbf{x}_G$ is precisely the number of non-zero entries in $\mathbf{x}$. This suggests that postprocessing $\tilde{\mathbf{x}}_G$ to ensure that the counts are non-decreasing will lead to a significant reduction of error for sparse datasets. We evaluate this strategy  in Section~\ref{sec:experiments}.

\subsubsection{Marginals under $G^1_{k^d}$}
Let us consider the case of two dimensions, where the marginals are row and column sums (see Figure~\ref{fig:2Dline-c} for reference). First, consider only the column sums. For any single column sum query, the transformed query is difference between the sum of edges to the right of the column and and the sum of the edges to the left of the column. Thus, answering all the column sums in $\mathbf{x}$ requires (a) computing the sums of all the columns of edges in $\mathbf{x}_G$, and (b) computing the difference between adjacent sums  to get the column sums in $x$. The strategy for row sums is similar, except that we consider all the vertical edges. 

We make two important observations. First, the transformed row queries and the transformed column sum queries pertain to disjoin sets of edges (vertical and horizontal, resp). Hence, they can each be answered using $\epsilon$-differential privacy (parallel composition). This holds even in $d$ dimensions. Second, the strategy we outlined for answering column (or row) sums seems exactly the same as our strategy for answering histogram queries under $G^1_k$ after appropriate marginalization of both the database and the graph! We formalize this intuition using the following notion of {\em policy graph marginalization}.

\begin{definition}[Marginalization]
Let $\mathbf{x}$ be a database, and $\mathbf{W}$ be a workload. We say that the columns in $\mathbf{W}$ corresponding to domain elements  $u,v \in \dom$ can be {\em marginalized} if they are identical. 
\end{definition}
Note that for the column sums workload, all points $(u,v)$ and $(u',v)$ would correspond to identical columns in the workload. We define $\mathbf{x}_{(u+v)}$ to be a dataset on domain $\dom - \{v\}$, where $\mathbf{x}_{(u+v)}[u] = \mathbf{x}[u] + \mathbf{x}[v]$. We define $\mathbf{W}_{(u+v)}$ to be the workload $\mathbf{W}$ with the column corresponding to $v$ dropped. For a graph $G = (V, E)$ and $u,v \in v$, we denote by $G_{(u+v)}$ the graph that merges nodes $u$ and $v$ into a single node.

\begin{lemma}\label{lem:graph-marg}
Let $G$ be a policy graph, and $\mathbf{x}$ be a database. Let $\mathbf{W}$ be a workload where $u, v \in \dom$ can be marginalized. Then a mechanism $\mathcal{M}$ for answering $\mathbf{W}$ on $\mathbf{x}$ satisfying $(\epsilon, G)$-Blowfish policy is also a mechanism for answering $\mathbf{W}_{(u+v)}$ on $\mathbf{x}_{(u+v)}$ satisfying $(\epsilon, G_{(u+v)})$-Blowfish policy
\end{lemma}
\begin{proof}(sketch)
It is easy to show that $\mathbf{W}\mathbf{x} = \mathbf{W}_{(u+v)}\mathbf{x}_{(u+v)}$. It is also easy to show that $\mathbf{y}$ and $\mathbf{z}$ are neighbors according to $G$ only if $\mathbf{y}_{(u+v)}$ and $\mathbf{z}_{(u+v)}$ are neighbors according to $G_{(u+v)}$. This gives us the required result.
\end{proof}

Therefore, for releasing a marginal on a single dimension, we can marginalize the workload, database and the graph by merging (or summing up) all the nodes in each column into a single node. The resulting workload is a histogram, resulting database is the set of column sums and the resulting graph is a line graph $G^1_k$! So we can use the strategy for releasing histograms for releasing each marginal. We believe policy graph marginalization would be very helpful to simplify the graph (and hence the transformed database/workload) when queries pertain to only a subset of the attributes. 

\eat{ %%% START EAT
Our strategy for answering histograms under $G^1_k$ is very similar to that of answering range queries in $G^1_k$. 
We propose the following algorithm for answering this workload under the line graph.

\begin{algorithm}[t]
  \caption{Histogram queries.}
  \label{alg:1D-marginal}
  \begin{algorithmic}[1]
    \Require
      \Statex $\mathbf{W}$ is a workload of range queries, $\mathbf{x}$ is a database.
    \Function{Hist}{$\mathbf{W},\mathbf{x}$}
      \Let{$\mathbf{x}_{G}$}{$\mathbf{P}_{G^1_k}^{-1}\mathbf{x}$  {\small {\em // prefix sums from $\mathbf{x}$}}}
      \Let{$\tilde{\mathbf{x}}_{G}$}{Differentially private estimate for $\mathbf{x}_{G}$}
      \Let{$\mathbf{W}_{G}$}{$\mathbf{WP}_{G^1_k}$ {\small {\em // differences between prefix sum pairs}} }
      \State \Return $\mathbf{W}_{G} \tilde{\mathbf{x}}_{G^1_k}$
    \EndFunction
  \end{algorithmic}
\end{algorithm}
Unlike the range queries, the transformed histogram workload is not any easier to answer than the original workload.
Every query has two nonzero entries instead of one.
Therefore, data-independent techniques will not help us.
However, data-dependent techniques may still help: the entries in $\mathbf{x}_G$ are ordered, while the entries in $\mathbf{x}$ are not.
We present this result in Section~\ref{sec:experiments}.

We next investigate 1D marginals over two-dimensional data under $G^1_{k^2}$.
} %%% END EAT




==> graphs.tex <==
%!TEX root = paper.tex

We compare naive methods for satisfying Blowfish privacy to data-dependent versions of the algorithms we develop.
We answer three workloads: 10,000 random one-dimensional range queries, 10,000 random two-dimensional range queries, and the histogram workload.
For each workload, we aim to satisfy $(\epsilon,G^1_k)$-Blowfish privacy and $(\epsilon,G^1_{k^2})$ for one-dimensional and two-dimensional data, respectively.
All experiments were performed using values of 1 and .1 for epsilon.
In all cases, error is reported as average $L_2$.

We answer one dimensional range queries using three different strategies.
First, we answer the queries using the DAWA framework \cite{li14:dawa}.
Next, we transform the workload by $\mathbf{P}_{G^1_k}$ and answer a histogram by adding Laplace noise to each query.
Each query is then reconstructed from two histogram queries, as described in the previous section.
The results for this strategy are labeled ``Transformed'' in the plot.
Finally, we note that transformation by $\mathbf{P}_{G^1_k}$ necessarily constrains $\mathbf{x}_{G^1_k}$ to be ordered.
We enforce this ordering after adding Laplace noise using the results of \cite{vldb:HayRMS10}.
These results are labeled ``Transformed + ConsistentEst'' in the plot.

We answer the histogram using similar strategies.
In this case, note that the transformed workload does not seem any easier to answer than the original workload, as it was in the case of range queries.
However, $\mathbf{x}_{G^1_k}$ is again ordered, and this allows us to answer with much lower error in some cases.

Finally, we compare two strategies for answering two dimensional range queries.
First, we answer the range queries using the DAWA framework.
Next, we transform the workload and database.
As shown in the previous section, each query in this transformed workload of 4 one-dimensional range queries.
We answer this query using the DAWA framework.
One weakness of this approach is that the transformed database $\mathbf{x}_{G^1_k}$ will generally not be sparse, even if $\mathbf{x}_{G^1_k}$ is sparse.
However, our strategy of transforming the instance before applying DAWA still outperforms the more naive approach.


==> omitted_proofs.tex <==
%\mmerror*
%\input{proof_mmerror}

%\sensitivityEquivalence*
%\input{proof_sensitivityEquivalence}

\neighborEquality*
\input{proof_neighborEquality}

\querytransformation*
\input{proof_query-transformation}

\independent*
\input{proof_independent}

\inverse*
\input{proof_inverse}


\blowfishSVDB*
\input{proof_blowfishSVDB}

\subgraph*
\input{proof_subgraph}

\rangeTheta*
\input{proof_rangeTheta}


==> proof_blowfishEquality.tex <==
\begin{proof}

  Construct $\mathcal{M}$ from $\mathcal{M}_G$ as follows:
  \begin{enumerate}
    \item On input $\mathbf{W},\mathbf{x}$, let $\mathbf{W}_G = \mathbf{WP}_G$ and let $\mathbf{x}_G = \mathbf{P}_G^{-1}\mathbf{x}$.
    \item Return $\mathcal{M}_G(\mathbf{W}_G,\mathbf{x}_G)$.
  \end{enumerate}
  Mechansim $\mathcal{M}$ satisfies $(\epsilon,G)$-Blowfish privacy by Lemma~\ref{lem:neighborEquality}.
  Next, we have that $\mathcal{M}_G(\mathbf{W}_G,\mathbf{x}_G) = \mathcal{M}(\mathbf{W},\mathbf{x})$.
  Additionally, the true answers to each mechanism are equvialent, since
  \begin{equation*}
    \mathbf{W}_G\mathbf{x}_G = \mathbf{W}\mathbf{P}_G\mathbf{P}_G^{-1}\mathbf{x} = \mathbf{W}\mathbf{x}.
  \end{equation*}
  Therefore,
  \begin{equation*}
    \mathrm{ERROR}^G_{\mathcal{M}}(\mathbf{W},\mathbf{x}) = \mathrm{ERROR}_{\mathcal{M}_G}(\mathbf{W}_G,\mathbf{x}_G).
  \end{equation*}
  Construct $\mathcal{M}_G$ from $\mathcal{M}$ as follows:
  \begin{enumerate}
    \item On input $\mathbf{W}_G,\mathbf{x}_G$, let $\mathbf{W} = \mathbf{WP}_G^{-1}$ and let $\mathbf{x} = \mathbf{P}_G\mathbf{x}_G$.
    \item Return $\mathcal{M}(\mathbf{W},\mathbf{x})$.
  \end{enumerate}
  Proofs of differential privacy and error equivalence are similar to the first direction.

\end{proof}


==> proof_blowfishError.tex <==
\begin{proof}
  This proof is nearly identical to the proof of Theorem~\ref{thm:mm-error} from \cite{pods:LiHRMM10} and \cite{edbt:chaoli13}, except that we use the policy specific sensitivity. For instance, in the case of $\mathrm{ERROR}_{(\mathcal{G},\mathbf{A})}^G(\mathbf{W})$ instead of obtaining $\sigma^2 = P(\epsilon,\delta)\Delta_\mathbf{A}^2$ as we did in the original proof, we obtain $\sigma^2=P(\epsilon,\delta)(\Delta_\mathbf{A}(G))^2 = P(\epsilon,\delta)\Delta_{\mathbf{A}_G}^2$. This follows directly from the fact that we have defined $\sigma$ using the policy specific sensitivity.
\end{proof}


==> proof_blowfishSVDB.tex <==
\begin{proof}
  From the results of \cite{edbt:chaoli13} we have 
  \begin{equation*}
    \mathrm{ERROR}_\mathcal{M}(\mathbf{W}_G)\ge P(\epsilon,\delta)\frac{1}{n_G}(\lambda_1+\ldots+\lambda_s)^2
  \end{equation*}
  for any matrix mechanism $\mathcal{M}$, where $P(\epsilon,\delta) = \frac{2\log(2/\delta)}{\epsilon^2}$, $\lambda_1,\ldots,\lambda_s$ are the singular values of $\mathbf{W}_G$, and $n_G$ is the number of columns of $\mathbf{W}_G$. 
  The result then follows immediately from Corollary~\ref{cor:blowfish-lower-bound}.
\end{proof}


==> proof_domainEquality.tex <==
\begin{proof}
  First, assume $\mathbf{BA}=\mathbf{W}$. Then
  \begin{align*}
    &\mathbf{BAP}_G = \mathbf{WP}_G \ \ \implies \ \
    \mathbf{BA}_G = \mathbf{W}_G
  \end{align*}
  
  Next, assume $\mathbf{BA}_G = \mathbf{W}_G$. Then
  \begin{eqnarray*}
    \mathbf{BAP}_G = \mathbf{WP}_G  & \implies & 
    \mathbf{BAP}_G\mathbf{P}_G^{-1} = \mathbf{WP}_G\mathbf{P}_G^{-1} \\
    & \implies & 
    \mathbf{BA}=\mathbf{W}
  \end{eqnarray*}
  Additionally, from Lemma \ref{lem:moore} we have that $\mathbf{WA}^+$ is a solution to $\mathbf{BA} = \mathbf{W}$, and $\mathbf{W}_G\mathbf{A}^+$ is a solution to $\mathbf{BA}_G = \mathbf{W}_G$. Because these equations have the same solution space, $\mathbf{WA}^+$ is a solution to $\mathbf{BA}_G = \mathbf{W}_G$ and $\mathbf{W}_G\mathbf{A}^+$ is a solution to $\mathbf{BA} = \mathbf{W}$.
\end{proof}


==> proof_errorEquivalence.tex <==
\begin{proof}
  This follows immediately from the following two facts from Theorem~\ref{thm:blowfishEquality} for both  ${\cal Z} = {\cal L}$ and ${\cal Z} = {\cal G}$: 
  \begin{align*}
    \mathrm{ERROR}_{({\cal Z}, \mathbf{A})}^G(\mathbf{W}) &= \mathrm{ERROR}_{({\cal Z}, \mathbf{A}_G)}(\mathbf{W}_G) \\
    \mathrm{MINERROR}_{{\cal Z}}(\mathbf{W}_G) &= \mathrm{MINERROR}_{{\cal Z}}^G(\mathbf{W}) 
\qed
  \end{align*}
\end{proof}


==> proof_independent.tex <==
\begin{proof}
  This is just a concise way of stating the following facts:
  \begin{itemize}
    \item If $m > n$, then $\mathbf{M}$ cannot have a right inverse. 
    \item If $m = n$, then $\mathbf{M}$ has both a left and right inverse if and only if its determinant is nonzero, which is true if and only if the matrix is full rank. 
    \item If $m < n$, then $\mathbf{M}$ has a right inverse if and only if it is full rank.
  \end{itemize}
\end{proof}


==> proof_inverse.tex <==
\begin{proof}
  Let $\mathbf{P}_{C_i}$ be the row projection of $\mathbf{P}_G$ that contains all the rows corresponding to vertices in $C_i$.
  Consider $\mathbf{q}$, a row of $\mathbf{P}_{C_i}$.
  $\mathbf{q}$'s only nonzero entries correspond to edges in $C_i$.
  That is, $\mathbf{q}'$ cannot be written as a combination of rows that are not in $\mathbf{P}_{C_i}$ (since these rows will always have zeros in the entires corresponding to $\mathbf{q}$'s nonzero entries.
  Therefore, the following is enough:
  We first show that any component $C_i$ produces a $\mathbf{P}_{C_i}$ of rank $m_i-1$ where $m_i$ is the number of rows of $\mathbf{P}_{C_i}$. We then remove a row of $\mathbf{P}_{C_i}$, and show that this modification does not change the rank. We are then left with a $\mathbf{P}_{C_i}'$ with $m_i-1$ rows and rank $m_i-1$. So, the modified $\mathbf{P}_{C_i}'$ will be full rank.
  Once repeated for all components, we are left with a $\mathbf{P}_G'$ which has $m-c$ rows (where $m$ is the number of rows of $\mathbf{P}_G$ and $c$ is the number of components of $G$), which has rank $m-c$.

  Every component $C_i$ has a spanning tree $T_i$. Note that $\mathbf{P}_{T_i}$ is a column projection of $\mathbf{P}_{C_i}$, so to show $\mathbf{P}_{C_i}$ has rank $m_i-1$, it is sufficient to show that $\mathbf{P}_{T_i}$ has rank $m_i-1$.
  Every tree has at least two degree $1$ nodes. Let $v$ be one such node. The corresponding row of $\mathbf{P}_{T_i}$ has all zeros except for a single $1$ or $-1$. Let $\mathbf{e}_v$ be the value (row vector) of row $v$. Let the $k$th column be the one corresponding to the single nonzero element of $\mathbf{e}_v$. Other than row $v$, there is unique row $u$ which has a nonzero value in column $k$. Let $\mathbf{r}_u$ be the value of row $u$ with a zero in column $k$ and identical in all other values.

  Consider $\mathbf{P}_{T_i-v}$. This matrix will differ from $\mathbf{P}_{T_i}$ in the following ways: $\mathbf{P}_{T_i-v}$ will have all zeros in column $k$ and be missing row $v$. Additionally, the new value of row $u$ will be $\mathbf{r}_u$. Note that the value of row $u$ in $\mathbf{P}_{T_i}$, $\mathbf{e}_u$ can be written as $\mathbf{e}_u = \mathbf{r}_u-\mathbf{e}_v$. All rows in $\mathbf{P}_{T_i}$ other than $\mathbf{e}_u$ are linearly independent of $\mathbf{e}_v$. Therefore, every row in $\mathbf{P}_{T_i}$ can be written as a linear combination of a row in $\mathbf{P}_{T_i-v}$, and possibly $\mathbf{e}_v$. This means that $\mathrm{rank}(\mathbf{P}_{T_i})=1+\mathrm{rank}(\mathbf{P}_{T_i-v})$. $\mathbf{P}_{T_i-v}$ is also a tree, so we proceed inductively. The base case of this induction is a tree with only one edge, and this corresponds to a matrix of rank $1$. Therefore, $\mathbf{P}_{C_i}$ has rank $m_i-1$.

  Note that the $m_i-1$ rows we remove during the induction are all linearly independent, and the row corresponding the final vertex left over can be written as a linear combination of these $m_i-1$ rows. However, when we initially picked vertex $v$ of degree $1$, we had two choices for $v$, since any tree has two vertices of degree $1$. Since we have two choices at each inductive step, it is possible to pick any vertex we wish to end up with on the last step of the induction. That is, not only is does $\mathbf{P}_{C_i}$ have rank $m_i-1$, \textit{every} set of $m_i-1$ rows of $\mathbf{P}_{C_i}$ is linearly independent.

  Next, we have assumed that some column of $W$ corresponding to a vertex in $C_i$ is all zeros. This means that we may remove the corresponding row of $\mathbf{P}_{C_i}$ without changing $\mathbf{W}_G$. Because every set of $m_i-1$ rows of $\mathbf{P}_{C_i}$ is linearly independent, removing one row leaves us with $m_i-1$ rows, all of which are linearly independent.
\end{proof}


==> proof_mmerror.tex <==
\begin{proof}
  First part is given in \cite{edbt:chaoli13}. \todo{need to give proof sketch of the second part}.
\end{proof}


==> proof_neighborEquality.tex <==
\begin{proof}
  Consider $\mathbf{P}_G\mathbf{x}-\mathbf{P}_G\mathbf{z}$.
  Since $\mathbf{x}$ and $\mathbf{z}$ are neighbors, $\mathbf{x}-\mathbf{z} = \mathbf{\hat{i}}$, where $\mathbf{\hat{i}}$ is a vector with a single non-zero entry, which is 1.
  $\mathbf{P}_G\mathbf{\hat{i}}$ is a single column of $\mathbf{P}_G$.
  Therefore, either
  \begin{enumerate}
    \item $\mathbf{P}_G\mathbf{x}$ and $\mathbf{P}_G\mathbf{z}$ differ in two entries, each difference is just 1, and there is an edge between the two corresponding domain elements in $G$, or
    \item $\mathbf{P}_G\mathbf{x}$ and $\mathbf{P}_G\mathbf{z}$ differ in one entry, the difference is 1, and there is an edge between the corresponding element of $G$ and $\bot$.
  \end{enumerate}
  In either case, $\mathbf{P}_G\mathbf{x}$ and $\mathbf{P}_G\mathbf{z}$ are neighbors according to G.
  The proof in the other direction is similar.
\end{proof}


==> proof_query-transformation.tex <==
\begin{proof}
  Each entry $c$ of $\mathbf{q}_G$ satisfies $c = u - v$ where $u,v$ are entries in $\mathbf{q}$ and $(u,v) \in E$. $c$ is nonzero exactly when $u \ne v$, or equivalently, when
  \begin{equation*}
    |\left\{ u,v \right\} \cap \left\{ v_1,\dots,v_k \right\}| = 1. \qedhere
  \end{equation*}
\end{proof}


==> proof_rangeTheta.tex <==
\begin{proof}
  Here, we prove the lower bound of the theorem.
  Recall from Example~\ref{ex:workloads} that the workload $\mathbf{C}_k$ on domain $[1,k]$ is defined as the set of range queries $\{\mathbf{q}(1,i) \mid \forall 1 \leq i \leq k\}$. We show a lower bound of $\Omega(k^2/\epsilon^2)$ for $\mathbf{R}_k$ under Blowfish policy $G^1_k$ in 3 steps,
  \squishlist
  \item Partition the set of range queries $\mathbf{R}_k$ into a set of cumulative histogram queries $\mathbf{C}_k \cup \mathbf{C}_{k-1} \cup \ldots \cup \mathbf{C}_1$, each operating on a subset of the domain.
  \item Any strategy for answering $\mathbf{R}_k$ under $G^1_k$ incurs no less error than the sum of the errors incurred for the optimal Blowfish strategy for answering each $\mathbf{C}_i$, $i \in [k]$ under $G^1_i$ on the appropriate domain.
  \item  $\mathrm{ERROR}_\mathcal{M}^{G^1_k}(\mathbf{C}_k)  \ = \ \Omega(k/\epsilon^2) \quad \forall \mathcal{M}$. Thus, 
  \begin{align*}
    \mathrm{ERROR}_\mathcal{M}^{G^1_k}(\mathbf{R}_k) &\geq \sum_{i=1}^k\mathrm{ERROR}_\mathcal{M}^{G^1_i}(\mathbf{C}_i) \\
    &= \Omega(k^2/\epsilon^2) \quad \forall \mathcal{M}
  \end{align*}
  \squishend
  For the first step, if the domain $\dom = [k]$, then $\mathbf{R}_k$ is the set of queries $\{\mathbf{q}(i,j) \mid 1 \leq i \leq j \leq k\}$. This can be partitioned into disjoint sets of queries $\mathbf{S}_i = \{\mathbf{q}(i, j) \mid \forall j \mbox{ s.t. } i \leq j \leq k\}$. $\mathbf{S}_i$ is identical to the $\mathbf{C}_{k-i+1}$ workload on the domain $\{i, i+1, \ldots, k\}$.

  Next, note that $G^1_k$ restricted to the subdomain $\{i, i+1, \ldots, k\}$ correspond also to line graph $G^1_{k-i+1}$. Thus, it is enough to lower bound the sum of the minimum errors for answering each $\mathbf{C}_i$ under $G^1_i$, for $i \in [k]$.  

  By Corollary~\ref{cor:blowfish-lower-bound}, the lower bound on the error for $\mathbf{C}_k$ with respect to $G$ depends on the error under differential privacy of $\mathbf{C}_k \cdot P_{G^1_k}$, which is equal to the identity matrix $\mathbf{I}_{k-1}$ (see Example~\ref{ex:fullrank} on page \pageref{ex:fullrank}). Thus, we have
  \[\mathrm{ERROR}_\mathcal{M}^{G^1_k}(\mathbf{C}_k)  \ = \ \Omega(k/\epsilon^2) \quad \forall \mathcal{M}\]
  which competes the lower bound proof.

\end{proof}


==> proof_sensitivityEquivalence.tex <==
\begin{proof}
  \begin{equation*}
    \Delta_{(p,\mathbf{W})}(G) = \max_{(\mathbf{x},\mathbf{x}')\in N(G)}\norm{\mathbf{Wx} - \mathbf{Wx}'}_p
  \end{equation*}
  By the definition of neighbors, $\mathbf{x}$ and $\mathbf{x}'$ differ in two counts (an entry has been switched from one domain value to another). Let these be domain values be $i$ and $j$, and let $x_i$, $x_j$, $x'_i$, and $x'_j$ be their counts. So, $x_i = x'_i + 1$ and $x_j = x'_j - 1$. So, $\mathbf{Wx} - \mathbf{Wx}' = \mathbf{x} - \mathbf{x}'$. Additionally, by the definition of neighbors, $(i,j)$ must be an edge in $G$. Therefore, column there is a column in $\mathbf{P}_G$ which has a $1$ and $-1$ at $i$ and $j$. So, $\mathbf{x}-\mathbf{x}'$ is a column of $\mathbf{W}\mathbf{P}_G = \mathbf{W}_G$. So,
  \begin{equation*}
    \Delta_{(p,\mathbf{W})}(G) = \max_{\mathbf{v}_i\in\text{cols}(\mathbf{W}_G)}\norm{\mathbf{v}_i}_p
  \end{equation*} 
\end{proof}


==> proof_subgraph.tex <==
\begin{proof}
  Assume $D$ and $D'$ are neighboring databases under policy graph $G$. Then $D = A \cup \left\{ x \right\}$ and $D' = A \cup \left\{ y \right\}$ for some database $A$, and $(x,y) \in E$. From our assumption, $x$ and $y$ are connected by a path in $G'$ of length at most $\ell$. Therefore, there exist a sequence of vertices $x=v_1,\dots,v_j = y$ such that $(v_i, v_{i+1}) \in E$ and $j<\ell$. Further, $A \cup \left\{ v_i \right\}$ and $A \cup \left\{ v_{i+1} \right\}$ are neighbors under policy graph $G'$. Therefore, we have
  \begin{equation*}
    \mathrm{Pr} [\mathcal{M}(A \cup \left\{ v_i \right\}) \in S] \le e^\epsilon \cdot \mathrm{Pr} [\mathcal{M}(A \cup \left\{ v_{i+1} \right\}) \in S].
  \end{equation*}
    Composing over all $1 \le i \le j$ gives
  \begin{equation*}
    \mathrm{Pr} [\mathcal{M}(A \cup \left\{ x \right\}) \in S] \le e^{\epsilon \cdot \ell} \cdot \mathrm{Pr} [\mathcal{M}(A \cup \left\{ y \right\}) \in S],
  \end{equation*}
  as desired.
\end{proof}


==> proof_twodimrange_theta_figs.tex <==
\begin{figure}[b!]
  \centering
  \includegraphics[scale=1.4]{../Figures/2Dtheta_range_query}
  \caption{A two dimensional range query superimposed on $\mathbf{G}^\theta_{k^2}$. The graph is divided into squares with side length $\theta/2$. The red vertices fall at corners of the square.}
  \label{fig:2dtheta-range-query}
\end{figure}

\begin{figure}[b!]
  \centering
  \includegraphics[scale=1.4]{../Figures/2Dtheta_range_strat_external}
  \caption{We highlight in red all the external edges on the transformed query. These edges form four one dimensional ranges. Which can be answered according to the strategy described in Section~\ref{sec:ddimrange}.}
  \label{fig:range-strat-external}
\end{figure}

\begin{figure}[b!]
  \centering
  \includegraphics[scale=1.4]{../Figures/2Dtheta_range_strat_internal}
  \caption{The remaining edges in the transformed query are all internal edges. These edge ordered by their non-red endpoints. These non-red endpoints make up four two dimensional ranges, illustraed here with red dashed boxes. Recall that in each square, all vertices are adjacent only to the upper right corner of the square. Because we order the edges according to these non-red vertices, the edges will also form four two dimensional range queries. Note that these range queries are constrained to $\theta$ in one dimension. In general, the $d$ dimensional range queries produced in this way will be constrained to size $\theta$ in one dimension, the dimension orthogonal to the corresponding face of the original range query.}
  \label{fig:range-strat-internal}
\end{figure}


==> rangeSVD.tex <==
\begin{figure}[h!]
  \centering
  \begin{subfigure}{.49\textwidth}
    \centering
    \includegraphics[width=.8\textwidth]{../Figures/SVDBoundPlots/plots/allrange}
    \caption{All Ranges}
    \label{fig:allrange-lb}
  \end{subfigure}
  \begin{subfigure}{.49\textwidth}
    \centering
    \includegraphics[width=.8\textwidth]{../Figures/SVDBoundPlots/plots/2drange}
    \caption{All $2$-dimensional Ranges}
    \label{fig:2dranges-lb}
  \end{subfigure}
  \caption{Lower bounds for range query workloads under Blowfish policies.}
  \label{fig:lb}
\end{figure}

We illustrate the lower bound given in Corollary~\ref{cor:blowfishSVDB} for 1-dimensional ($\mathbf{R}_k$) and 2-dimensional ($\mathbf{R}_{k^2}$) range queries satisfying $(\epsilon, \delta, G^\theta_k)$-Blowfish privacy and $(\epsilon, \delta, G^\theta_{k^2})$-Blowfish privacy respectively. %for various $\theta$'s.

Figures~\ref{fig:allrange-lb} and \ref{fig:2dranges-lb} illustrate the relationship between the lower bound on error and size of the domain for $\mathbf{R}_k$ and $\mathbf{R}_{k^2}$ respectively. We plot the original lower bound for unbounded differential privacy (from \cite{edbt:chaoli13}) and the new lower bounds we derived for Blowfish policies $G_k^{\theta}$ and $G^\theta_{k^2}$ for various values of $\theta$. Additionally, we show a lower bound for bounded differential privacy, which is obtained by using the complete graph (on $\dom$) as the policy graph. 

For the one dimensional range query workload we see that minimum error under unbounded differential privacy increases faster than the minimum error under $G^{\theta}_k$ for sufficiently large domain sizes.  For two dimensional ranges, error under Blowfish policy $G^{\theta}_{k^2}$ is only better than unbounded differential privacy for $\theta=1$. However, all values of $\theta$ perform better than bounded differential privacy. Note that for sets of linear queries, it is possible for the sensitivity of a workload under bounded differential privacy to be twice the sensitivity of the workload under unbounded differential privacy, and thus have up to 4 times more error. Characterizing analytical lower bounds for these workloads and policies is an interesting avenue for future work.


==> range_figures.tex <==

\begin{figure*}[h!]
  \centering
  \begin{subfigure}[t]{.48\textwidth}
    \centering
    \includegraphics[width=.7\textwidth]{../Figures/range/2Dtheta_graph}
    \caption{$G^2_{5^2}$, each vertex is connected to other vertices within $L_1$ distance 2 on the grid.}
    \label{fig:2Dtheta-a}
  \end{subfigure}
  \quad
  \begin{subfigure}[t]{.48\textwidth}
    \centering
    \includegraphics[width=\textwidth]{../Figures/range/2Dtheta_subgraph}
    \caption{A section of $\mathbf{H}^4_{k^2}$. Internal edges are light blue and external edges are black.}
    \label{fig:2Dtheta-b}
  \end{subfigure}
  \par\bigskip\bigskip
  \begin{subfigure}[t]{.48\textwidth}
    \centering
    \includegraphics[width=\textwidth]{../Figures/range/2Dtheta_query_external}
    \caption{A 2D range query superimposed on the graph. Instead of showing all vertices, we show the divisions in $\theta/2$ blocks. Within each block, all vertices would be connected to the upper right corner. The grid of lines shows all the external edges. Highlighted in purple are the external edges which satisfy Lemma~\ref{lem:query-transformation} and therefore appear in the transformed query.}
    \label{fig:2Dtheta-c}
  \end{subfigure}
  \quad
  \begin{subfigure}[t]{.48\textwidth}
    \centering
    \includegraphics[width=\textwidth]{../Figures/range/2Dtheta_query_internal}
    \caption{The shaded rectangles show the sets of vertices corresponding to the internal edges which satisfy Lemma~\ref{lem:query-transformation}. There are 4 such rectangles, and for each one either the height or length is bounded by $\theta$. Note that there are other ways in which we could divide the shaded region into 4 rectangles, we arbitrarily chose one. Our strategy is to answer all range queries over each row squares, and each column of squares.}
    \label{fig:2Dtheta-d}
  \end{subfigure}
  \caption{Transforming queries in $\mathbf{R}_{k^2}$ under $G^\theta_{k^2}$.}
  \label{fig:2Dtheta}
\end{figure*}


==> rangequeries.tex <==
%!TEX root = paper.tex
In this section, we derive upper bounds on the error (and in some cases near optimal strategies) under the extended matrix mechanism framework for answering multidimensional range query workloads ($\mathbf{R}_k$ and $\mathbf{R}_{k^d}$) under $(\epsilon, G)$-Blowfish privacy for policies described by $G^\theta_k$ and $G^\theta_{k^d}$, respectively (defined in Section~\ref{sec:lower-range}). We first propose strategies for answering $\mathbf{R}_k$ and $\mathbf{R}_{k^d}$ under $G^1_k$ and $G^1_{k^d}$, respectively, using  transformational equivalence (Theorem~\ref{thm:blowfishEquality}). We then derive upper bounds for the more general $G^\theta_k$ and $G^\theta_{k^d}$ using a general technique called {\em subgraph approximation}. We describe these two general techniques in detail in Section~\ref{sec:strategytechniques}, and derive near optimal strategies (and thus upper bounds on error) for one- and multi-dimensional range queries in Section~\ref{sec:one-range-upper} and Section~\ref{sec:d-range-upper}, resp.

\begin{figure}[t]
  \centering
  \begin{tabular}{| c | c c | c | }
    \hline
    \multirow{2}{*}{$\mathbf{W}$} & \multicolumn{3}{|c|}{\textbf{Error per query}} \\
    \cline{2-4}
    & \multicolumn{2}{|c|}{\small \textbf{Blowfish}} & {\small \textbf{$\epsilon$-Diff. Privacy \cite{icde:XiaoWG10}}}\\
    \hline
    \multirow{2}{*}{$\mathbf{C}_k$} & $G^1_k$ & $\Theta(1/\epsilon^2)$ & \multirow{2}{*}{$O(\log^3 k / \epsilon^2)$} \\
     & $G^{\theta}_k$ & $O(\log^3{\theta}/\epsilon^2)$ & \\
    \hline
    $\mathbf{R}_k$ & $G^1_k$ & $\Theta(1/\epsilon^2)$ & $O(\log^3 k / \epsilon^2)$ \\
    $\mathbf{R}_{k^2}$ & $G^1_{k^2}$ & $O(\log^3 k / \epsilon^2)$ & $O(\log^6 k / \epsilon^2)$  \\
    \hline
    \multirow{2}{*}{$\mathbf{R}_{k^d}$} & $G^1_{k^d}$ & $O(\frac{d^3 \log^{3(d-1)}k}{\epsilon^2})$ & \multirow{2}{*}{$O(\log^{3d}k / \epsilon^2)$} \\
    & $G^\theta_{k^d}$ & $O(\theta^2\cdot \frac{d^3 \log^{3(d-1)}k}{\epsilon^2})$ &  \\
    \hline
  \end{tabular}
  \caption{Summary of results. $\mathbf{C}_k$ is the cumulative histogram workload with domain size $k$. $\mathbf{R}_{k^d}$ is the $d$ dimensional all range queries workload where each dimension has a domain size of $k$.}
  \label{fig:summary}
\end{figure}



\subsection{Techniques}\label{sec:strategytechniques}

To find optimal strategies, we can use the matrix mechanism \cite{pods:LiHRMM10} directly on $\mathbf{W_G} = \mathbf{W}\mathbf{P_G}$. However, the matrix mechanism is inefficient and $\mathbf{W}_G$ will potentially be much larger than $\mathbf{W}$ (especially when $G$ is dense). Instead, we use existing literature on (near) optimal strategies for differential privacy to find (near) optimal strategies for Blowfish. We next describe the two main techniques we use -- {\em transformational equivalence} and {\em subgraph approximation}. 

\subsubsection{Transformational Equivalence}\label{sec:equivalence-application}

Theorem~\ref{thm:blowfishEquality} shows that the error for workload $\mathbf{W}$ using strategy $\mathbf{A}$ under policy graph $G$ is equal to the error for $\mathbf{W}_G = \mathbf{W} \mathbf{P}_G$ using strategy $\mathbf{A}_G$ under both \todo{bounded and unbounded} differential privacy. Hence, we adopt the following general strategy:
%Ashwin: Do we need to say bounded and unbounded?? 

\squishlist
  \item Given $\mathbf{W}$, convert to $\mathbf{W_G} = \mathbf{W}\mathbf{P}_G$.
  \item Find some strategy $\mathbf{A}_G$ to answer $\mathbf{W}_G$ with low error under differential privacy.
  \item Use $\mathbf{A}_G\mathbf{P}_G^{-1}$ to answer $\mathbf{W}$.
\squishend

Based on Theorem~\ref{thm:blowfishEquality}, it is easy to show that if $\mathbf{A}$ can answer $\mathbf{W}_G$ with near optimal error, then $\mathbf{AP}^{-1}_G$ is a near optimal strategy for $\mathbf{W}$. 

\begin{restatable}{corollary}{errorEquivalence}\label{cor:errorEquivalence} 
  Let $c \geq 1$ be some real number. Let $G$ be a Blowfish policy graph, $\mathbf{W}$ be a linear workload and $\mathbf{A}$ be a strategy for answering the workload. Let $\mathbf{W}_G = \mathbf{WP}_G$ and $\mathbf{A}_G = \mathbf{AP}_G$. Then, $\mathrm{ERROR}^G_{(\mathcal{Z},\mathbf{A})}(\mathbf{W}) \leq c \cdot \mathrm{MINERROR}_\mathcal{Z}^G(\mathbf{W})$ if and only if $\mathrm{ERROR}_{(\mathcal{Z},\mathbf{A}_G)}(\mathbf{W}_G) \leq c \cdot \mathrm{MINERROR}_\mathcal{Z}(\mathbf{W}_G)$, for both $\mathcal{Z} =\mathcal{G}$ and $\mathcal{Z} = \mathcal{L}$.
\end{restatable}
\begin{proof}
  See Appendix.
\end{proof}


Note that when we directly find a strategy for $\mathbf{W}_G$, we call it $\mathbf{A}_G$. This way, we let $\mathbf{A}_G\mathbf{P}_G^{-1}$, which is a strategy for $\mathbf{W}$ with equivalent error, be called $\mathbf{A}$. Then we have $\mathbf{A}_G = \mathbf{A}\mathbf{P}_G$ which is consistent with the rest of the paper.

An important consequence of the above corollary (which we will use later) is that if we know an optimal strategy $\mathbf{A}_G$ (or $c = 1$ in the above Corollary) for answering $\mathbf{W}_G$ under differential privacy, the strategy $\mathbf{A}_G\mathbf{P}_G^{-1}$ is an optimal strategy for answering $\mathbf{W}$ under the Blowfish policy graph $G$. Theorem~\ref{thm:blowfishEquality} and Corollary~\ref{cor:errorEquivalence} allow us to leverage the rich literature on the matrix mechanism for differential privacy to design efficient mechanisms for answering workloads under Blowfish. We would like to point out that the error equivalence in Theorem~\ref{thm:blowfishEquality} and Corollary~\ref{cor:errorEquivalence} applies both to the total error as well as the error per query, since the number of queries in $\mathbf{W}$ and $\mathbf{W}_G$ are the same. 

\subsubsection{Subgraph Approximation}\label{sec:subgraph-approx}

Our technique from the previous section only works if $\mathbf{W}_G$ is well studied, or similar to well studied workloads. Although this is sometimes the case, depending on $G$, $\mathbf{W}_G$ may be very different from standard workloads. In this case, it is sometimes possible to sacrifice a constant factor $\ell^2$ in error to change $G$ to  a subgraph $G'$ such that $\mathbf{W}_{G'}$ is more similar to a well studied workload. $\ell$ is related to ratio of the distances between vertices in $G$ and $G'$. 

\begin{definition}[$\ell$-spanner]
A graph $G' = (V, E')$ is a $\ell$-spanner of $G = (V,E)$ if $E' \subset E$, and every pair $(u,v) \in E$ is connected by a path of length at most $\ell$ in $G'$. 
\end{definition}
\begin{restatable}{lemma}{subgraph}[Subgraph Approximation]\label{lem:subgraph} 
If $G'$ is an $\ell$-spanner of $G$, then for any workload $\mathbf{W}$, we have
\begin{equation*}
  \Delta_{(p,\mathbf{W})}(G') \leq \Delta_{(p,\mathbf{W})}(G)  \leq \ell \cdot  \Delta_{(p,\mathbf{W})}(G')
\end{equation*}
\end{restatable}
\begin{proof}
  See Appendix.
\end{proof}
%\input{proof_subgraph}


%Thus, if we can find a subgraph $G'$ of $G$ which approximates $G$, we can use $\mathbf{W}_{G'}$ and lose only an $\ell^2$ factor in the error. In some cases, we will be able to find a $\mathbf{W}_{G'}$ which is much easier to work with. Section~\ref{sec:mm-app-theta} gives an application of this idea.

We illustrate all these tools in the following sections. We focus on $(\eps, G)$-Blowfish privacy. Analogous upper bounds can be derived for $(\eps, \delta, G)$-Blowfish by using Gaussian noise; we defer details to a full version of the paper.

\subsection{1-Dimensional Range Queries}\label{sec:one-range-upper}
Recall that given a domain $\dom = [a,b]$ (where $k = b-a+1$), all queries in $\mathbf{R}_k$ correspond to intervals $[x,y]$, $a \leq x \leq y \leq b$.  Note that each of these queries can be written as a difference between two one-sided range queries $[a,y]$ and $[a,x]$. Thus, if we have a strategy for answering all queries in $\mathbf{C}_k$, we can reconstruct the answers to all queries in $\mathbf{R}_k$. 

In fact, we can show that using an optimal strategy for $\mathbf{C}_k$ to answer $\mathbf{R}_k$ is a $2$-approximate to the optimal strategy for $\mathbf{R}_k$. More formally, 
\begin{restatable}{theorem}{rkck}\label{thm:rkck}
Let $c \geq 1$ be a real number. Let $G$ be a Blowfish policy graph, and $\mathbf{A}$ be a $c$-approximate strategy for $C_k$ under policy $G$. That is, $\mathrm{ERROR}^G_{(\mathcal{L},\mathbf{A})}(\mathbf{C}_k) \leq c \cdot \mathrm{MINERROR}_\mathcal{L}^G(\mathbf{C}_k)$. Then, 
$$\mathrm{ERROR}^G_{(\mathcal{L},\mathbf{A})}(\mathbf{R}_k) \leq 2c \cdot \mathrm{MINERROR}_\mathcal{L}^G(\mathbf{R}_k)$$
\end{restatable}  
\begin{proof}

\end{proof}
%\subsection{Near Optimal Strategies for $\mathbf{C}_k$}\label{sec:ck-upper}

%We give strategies for answering the cumulative histogram workload, $\mathbf{C}_k$, where $k$ is the size of the domain. We begin by giving an optimal strategy for answering $\mathbf{C}_k$ under a line graph. Next, we use Lemma~\ref{lem:subgraph} to find a near optimal strategy for answering $\mathbf{C}_k$ under $G^{\theta}_k$. Additionally, we analyze the strategy that we produce for $\mathbf{C}_k$, and show why it produces near optimal error.

\subsubsection{$\mathbf{C}_k$ under the line graph}\label{sec:mm-app-line}
In Example~\ref{ex:sensitivity}, we showed that the policy specific global sensitivity of $\mathbf{C}_k$ under the line graph policy $G_k^{Line}$ is $1$. Thus it seems like the optimal strategy for answering $\mathbf{C}_k$ under line graph policy is to add independent noise (Laplace for $\epsilon$- and Gaussian for $(\epsilon,\delta)$- differential privacy) to each of the queries in $\mathbf{C}_k$ resulting in $\Theta(1/\epsilon^2)$ error for each of the counts in $\mathbf{C}_k$. We can formally prove that this is the optimal strategy using Corollary~\ref{cor:errorEquivalence}.

\begin{theorem}\label{thm:hist-line}
  Let $\mathbf{C}_k$ be the cumulative histogram workload, and let $G_k^{Line}$ be the line graph. Then $\mathbf{C}_k$ can be answered with $\Theta(1/\epsilon^2)$ error per query under $(\epsilon, G_k^{Line})$- as well as $(\epsilon, \delta, G_k^{Line})$-Blowfish privacy. Moreover, this is optimal.
\end{theorem}
\begin{proof}
  We first modify $\mathbf{C}_k$ and $P_{G^{Line}_k}$ as per Example~\ref{ex:fullrank}. The first row (query) in $\mathbf{C}_k$ is $Q_n$, which returns the number of elements in the database. Since this query is already known, we can replace it with all zeros. The first row and column of $\mathbf{C}_k$ can be eliminated, producing $\mathbf{C'}_k$ (which is the same as $\mathbf{C}_{k-1}$).  We remove the corresponding row (first) from $\mathbf{P}_{G^{Line}_k}$ to get $\mathbf{P'}_{G^{Line}_k}$. 

  Now, it is easy to check that $\mathbf{C'}_k\mathbf{P'}_{G^{Line}_k}$ is the identity matrix $\mathbf{I}_{k-1}$ (or the histogram query). The optimal strategy for answering the histogram query under differential privacy is to add independent noise to each of the counts; i.e., the optimal strategy is $\mathbf{I}_{k-1}$. Hence, from Corollary~\ref{cor:errorEquivalence}, the optimal strategy for answering  $\mathbf{C'}_k$ under the line graph policy is $\mathbf{I}_{k-1} \mathbf{P'}_{(G^{Line}_k)}^{-1} = \mathbf{C'}_k$. Thus the optimal strategy for answering the cumulative histogram workload under the line graph policy is to just use the Laplace (or Gaussian) mechanism. 
\end{proof} 

\begin{figure}[t]
\centering
\subfigure[Strategy matrices for $m=3$]{
\includegraphics[scale=0.3]{../Figures/thetagraph_matrices_v2}
\label{fig:thetagraph_matrices}
}
\subfigure[$\mathbf{S}_\theta$, for $\theta = 8$]{
\includegraphics[scale=0.375]{../Figures/Stheta}
\label{fig:Stheta}
}
\subfigure[Strategy $\mathbf{A}$ explained $(m=3, \theta = 8)$]{
\includegraphics[scale=0.3]{../Figures/cumulative_theta_strategy_cropped}
\label{fig:cumulative_theta_strategy}
}
\caption{Deriving the strategy for answering $\mathbf{C}^\theta_k$ under the discriminative secret graph $\hat{G}^\theta_k$}
\end{figure}

\xxx{
{\small
\begin{tabular}{cccccccc}
0 & 0 & 0 & 0 & 0 & 0 & 0 & 1\\
0 & 0 & 0 & 1 & 1 & 1 & 1 & 1\\
0 & 1 & 1 & 1 & 1 & 1 & 1 & 1\\
1 & 1 & 1 & 1 & 1 & 1 & 1 & 1\\
0 & 0 & 0 & -1 & -1 & -1 & -1 & 0\\
0 & 0 & 0 & -1 & -1 & 0 & 0 & 0\\
0 & 0 & 0 & 0 & 0 & -1 & -1 & 0\\
0 & 0 & 0 & -1 & 0 & 0 & 0 & 0\\
0 & 0 & 0 & 0 & -1 & 0 & 0 & 0\\
0 & 0 & 0 & 0 & 0 & -1 & 0 & 0\\
0 & 0 & 0 & 0 & 0 & 0 & -1 & 0\\
0 & -1 & -1 & 0 & 0 & 0 & 0 & 0\\
0 & -1 & 0 & 0 & 0 & 0 & 0 & 0\\
0 & 0 & -1 & 0 & 0 & 0 & 0 & 0\\
-1 & 0 & 0 & 0 & 0 & 0 & 0 & 0\\
\end{tabular} 
}
}

\subsubsection{$\mathbf{C}_k$ under $G^{\theta}_k$}\label{sec:mm-app-theta}
In Example~\ref{ex:sensitivity}, we also saw that the $L_1$ sensitivity of $\mathbf{C}_k$ under $G^{\theta}_k$ is $\theta$.  Thus, the Laplace mechanism that adds $Lap(\theta/\epsilon)$ noise ensures $\epsilon$-differential privacy with $2 \theta^2/\epsilon^2$ error per query. We can show a near optimal and efficient strategy for answering $\mathbf{C}_k$ under $(\epsilon, G^{\theta}_k)$-Blowfish privacy with noise that only has a polylogarithmic dependence on $\theta$ -- a much smaller error for large $\theta$.

\begin{theorem}\label{thm:hist-theta}
  Let $\mathbf{C}_k$ be the cumulative histogram workload, and let $G^{\theta}_k$ be the graph which connects all vertices within distance $\theta$ along a line. $\mathbf{C}_k$ can be answered with $O(\frac{\log^3{\theta}}{\epsilon^2})$ error per query under $(\epsilon, G^{\theta}_k)$-Blowfish privacy.
\end{theorem}
\begin{proof}
  We derive our strategy for answering $\mathbf{C}_k$ under a slightly different discriminative secret graph $\hat{G}^{\theta}_k$ (Fig~\ref{fig:graphs}), which is a spanning tree of $G_k^{\theta}$. Recall that in $G^\theta_k$ vertices $i$ and $j$ are connected if they are no more than $\theta$ apart (i.e., $|i-j| \leq \theta$). We construct $\hat{G}^{\theta}_k$ by connecting vertex $j$ to $i$ if $i - \theta \le j < i$ and $i$ is a multiple of $\theta$. We discard all other edges of $G_k^{\theta}$. Observe that for every edge $(u,v)$ in $G_k^{\theta}$, either $(u,v)$ already appears in $\hat{G}^{\theta}_k$, or $u$ and $v$ are connected by a path of length $3$. Thus by Lemma~\ref{lem:subgraph}, we can focus on designing a strategy for answering $\mathbf{C}_k$ under the spanning tree $\hat{G}^{\theta}_k$, and the error under $G_k^{\theta}$ is at most $9$ times the error under $\hat{G}^{\theta}_k$.

  Again like in Sec~\ref{sec:mm-app-line}, we consider $\mathbf{C'}_k = \mathbf{C}_{k-1}$, and the matrix $\mathbf{P'}_{\hat{G}_k^{\theta}}$ after dropping the first row from $\mathbf{P}_{\hat{G}_k^{\theta}}$. We now have both $\mathbf{C'}_k$ and $\mathbf{P'}_{\hat{G}_k^{\theta}}$ as $(k-1) \times (k-1)$ square full rank matrices. For ease of exposition, let $k = m \cdot \theta + 1$ for some integer $m$. Additionally, let $\theta  = 2^b$, $b \geq 0$. 

  To construct the near optimal strategy for $\mathbf{C'}_k$ under $\hat{G}_k^{\theta}$, consider $\mathbf{C'}_{\hat{G}_k^{\theta}} = \mathbf{C'}_k \mathbf{P'}_{\hat{G}_k^{\theta}}$. $\mathbf{C'}_{\hat{G}_k^{\theta}}$ is a $m\cdot \theta \times m \cdot \theta$ square matrix, where the $\theta \times \theta$ blocks along the diagonal each correspond to $\mathbf{C}_\theta^T$ ($\mathbf{C}_\theta^T$ is the transpose of $\mathbf{C}_\theta$) and all other entries are zero. Figure~\ref{fig:thetagraph_matrices} illustrates $\mathbf{C'}_{\hat{G}_k^{\theta}}$ for $m = 3$. Recent work has shown that a near optimal differentially private strategy (unbiased, linear and data independent) for answering $\mathbf{C}_\theta$ is the hierarchical strategy $\mathbf{H}_\theta$ \cite{stoc:DworkNPR10, pods:LiHRMM10, vldb:HayRMS10} (with error $O(\log^3(\theta)/\epsilon^2)$ per query). Thus we can answer $\mathbf{C'}_{\hat{G}_k^{\theta}}$ by answering every $\mathbf{C}_\theta^T$ in $\mathbf{C'}_{\hat{G}_k^{\theta}}$ using $\mathbf{H}_\theta$. Call this strategy $\mathbf{A}_{\hat{G}_k^{\theta}}$ (Fig~\ref{fig:thetagraph_matrices}).

  By Theorem~\ref{thm:blowfishEquality} we can answer $\mathbf{C'}_{m\cdot \theta}$ with $O(\log^3(\theta)/\epsilon^2)$ error per query under $\hat{G}^\theta_{m \cdot \theta+1}$ by using strategy $\mathbf{A}_{\hat{G}_k^{\theta}} \mathbf{P'}^{-1}_{\hat{G}_k^{\theta}}$. By Corollary~\ref{cor:errorEquivalence}, this must also be near optimal.
\end{proof}

To illustrate this further, we now provide an alternate proof for the above theorem which does not use Theorem~\ref{thm:blowfishEquality}. Instead, we examine $\mathbf{A} = \mathbf{A}_{\hat{G}_k^{\theta}} \mathbf{P'}^{-1}_{\hat{G}_k^{\theta}}$ directly, and show that is indeed a good strategy for $\mathbf{C'}_{k}$ under $\hat{G}_k^{\theta}$. Consequently, this is also a good strategy under policy graph $G_k^\theta$. 

Note that by construction, the policy specific sensitivity of $\mathbf{A}$ is the same as the global sensitivity of $\mathbf{A}_{\hat{G}_k^{\theta}}$; the $L_1$ sensitivity is $1 + \log \theta = 1 + b$. %, and the $L_2$ sensitivity is $\sqrt{1 + \ell}$. 
Thus, $\mathbf{C'}_k$ can be released privately by answering $\mathbf{A}$ using the Laplace mechanism with sensitivity $(1 + b)$. % or using the Gaussian mechanism with sensitivity $\sqrt{1+\ell}$. 

The strategy $\mathbf{A}$ is explained in Figure~\ref{fig:cumulative_theta_strategy}. $\mathbf{A}$ divides the domain $\dom = \{x_1, x_2, \ldots, x_{m\theta}\}$ into $m$ blocks of size $\theta$ and releases the same type of counts for each block. Consider the first block (and the counts are similar in the other blocks). $\mathbf{A}$ releases a set $C_\mathbf{A}$ of $1 + \log \theta = 1 + b$ cumulative counts $\{c_1, c_{1+2^{b-1}}, c_{1+2^{b-1}+ 2^{b-2}}, \ldots, c_{1+2^{b-1}+ 2^{b-2} + \ldots + 2^0}\}$, where $c_i$ is the sum of the counts of domain elements $x_i \ldots x_{m\theta}$. Additionally, $\mathbf{A}$ releases $\log \theta = b$ hierarchical counts $\mathbf{H}_{2^b-1}$, $\mathbf{H}_{2^b-2}, \ldots, \mathbf{H}_{1}$ for the cumulative counts $c_j$ that are not covered in the set $C_\mathbf{A}$. Using the example of $\theta = 8$ in Figure~\ref{fig:cumulative_theta_strategy}, $\mathbf{A}$ releases hierarchical counts $\mathbf{H}_4$ for elements $\{x_2, x_3, x_4, x_5\}$, $\mathbf{H}_2$ for elements $\{x_6, x_7\}$ and the count of $x_8$. It is easy to see that any cumulative count $c_j$ can be answered using at most $1 + b$ counts from $\mathbf{A}$. Thus, the total error for answering any single cumulative count is $O(\frac{(1 + \log \theta)^3)}{\epsilon^2})$ for $(\epsilon, \hat{G}^{\theta}_k)$-  and $(\epsilon, G^\theta_k)$-Blowfish privacy.


\subsection{Multidimensional Range Queries}\label{sec:d-range-upper}
%%% START EAT
\eat{We now give strategies for answering multidimensional AllRange queries under Blowfish. We defined multidimensional range query workloads and policy graph $G_{k^d}^\theta$ in Section~\ref{sec:lower-range}.
  

\subsubsection{$\mathbf{R}_k$ under $G^1_k$}\label{sec:onedimrange}

We begin with the case where $\theta$ is 1. In the one dimensional case, this will be a line graph.
\begin{theorem}\label{thm:range-1d}
  Workload $\mathbf{R}_k$ can be answered with $\Theta(1/\epsilon^2)$ error per query under $(\epsilon, G^1_k)$-Blowfish privacy.
\end{theorem}
\begin{proof}
  Consider one range query. The only places where the values of columns differ are at the two ends of the range. Therefore, multiplying by $G^1_k$ will result in a 1 or -1 at the ends of the range, unless the range started at one of the ends in which case the new query will be a single 1 or -1. $\mathbf{R}_{G^1_k} =\mathbf{R}_k \mathbf{P}_{G^1_k}$ will have ${k-1 \choose 2} + 2(k-1)$ rows. We can answer using strategy $\mathbf{I}_{k-1}$. Each query in $\mathbf{R}_{G^1_k}$ can be represented as a combination of at most 2 queries in $\mathbf{I}_{k-1}$, and the sensitivity of $\mathbf{I}_{k-1}$ is 1. Therefore, we can add $Lap(\frac{1}{\epsilon})$ noise to each row of $\mathbf{I}_{k-1}$, and each query in $\mathbf{R}_{G^1_k}$ can then be answered with at most $\frac{4}{\epsilon^2}$ error. Therefore, We can use strategy $\mathbf{I}_{k-1}\mathbf{P}_{G^1_k}^{-1}$ to answer $\mathbf{R}_{G^1_k}$ under $(\epsilon,G^1_k)$- Blowfish privacy. By Theorem~\ref{thm:blowfishEquality}, this will also have error $\Theta(1/{\epsilon^2})$ per query.
\end{proof}

%The total error for this workload will be $O(\frac{k^2}{\epsilon^2})$ since there are $O(k^2)$ queries in the workload. 
The best known strategy (with minimum error) for answering $\mathbf{R}_k$ under $\epsilon$-differential privacy is the Privelet strategy \cite{icde:XiaoWG10} with a much larger asymptotic error of $O(\log^3 k / \epsilon^2)$ per query. 
} 
%%% END EAT

\subsubsection{$\mathbf{R}_{k^d}$ under $G^1_{k^d}$}\label{sec:ddimrange}

Next, consider $d$ dimensional range queries. In this case, $G^1_{k^d}$ is a grid with $k^d$ vertices and $2d\cdot k^d$ edges. 
\begin{theorem}\label{thm:range-dd}
  Workload $\mathbf{R}_{k^d}$ can be answered with 
  \begin{equation*}
    O(\frac{d^3 \log^{3(d-1)}k}{\epsilon^2})
  \end{equation*}
  error per query under $(\epsilon, G^1_{k^d})$-Blowfish privacy.
\end{theorem}
\begin{proof}
  For some range query, the corresponding query in $\mathbf{R}_{G^1_{k^d}} = \mathbf{R}_{k^d} \mathbf{P}_{G^1_{k^d}}$ will essentially be the bounding box of the $d$ dimensional query hyperrectangle. That is, we can answer this query by answering all $2d$ $(d-1)$-dimensional ``faces'' of this bounding box under differential privacy. Therefore, we reduce the problem to answering $(d-1)$-dimensional range queries under differential privacy.

  To begin, we must split our epsilon budget $d$ ways in order to answer all range queries for each dimension. That is, we must answer $\mathbf{R}_{k^{d-1}}$ $d$ times, once for each dimension, under $\frac{\epsilon}{d}$-differential privacy. By composition, answering all of these workloads satisfies $\epsilon$-differential privacy. Using the Privelet framework \cite{icde:XiaoWG10}, we can answer a $d-1$ dimensional range query under $\frac{\epsilon}{d}$-differential privacy with $O(\frac{\log^{3(d-1)}k}{\epsilon^2/d^2}) = O(\frac{d^2 \log^{3(d-1)}k}{\epsilon^2})$. Let $\mathbf{B}$ be this strategy matrix: the noisy answers to all $d-1$-dimensional range queries for each of the $d$ dimensions. Each $d$-dimensional bounding box has $2d$ faces, and this bounding box query can therefore be answered using $2d$ rows from $\mathbf{B}$. Therefore, the error of answering each query in $\mathbf{R}_{G^1_{k^d}}$ is $O(2d\cdot \frac{d^2 \log^{3(d-1)}k}{\epsilon^2}) = O(\frac{d^3 \log^{3(d-1)}k}{\epsilon^2})$. By Theorem~\ref{thm:blowfishEquality}, $\mathbf{R}_{k^d}$ can be answered using strategy $\mathbf{B} \mathbf{P}_{G^1_{k^d}}^{-1}$ with $O(\frac{d^3 \log^{3(d-1)}k}{\epsilon^2})$ error per query under Blowfish policy graph $G^1_{k^d}$.
\end{proof}

If we consider $d$ to be a constant, then we get a $\Omega(\log^3{k})$ factor better error than differential privacy using Privelet \cite{icde:XiaoWG10}. In the two dimensional case, we achieve $O(\frac{\log^3 k}{\epsilon^2})$ error per query under Blowfish policy graph $G^1_{k^2}$, while Privelet achieves $O(\frac{\log^6 k}{\epsilon^2})$ error per query under differential privacy.

\subsubsection{$\mathbf{R}_{k^d}$ under $G^\theta_{k^d}$}
If we wish to consider $G^\theta_{k^d}$, we can use the same strategy as $G^1_{k^d}$ and our error will be worse by a factor of $\theta^2$. 
\begin{corollary}\label{cor:range-ddtheta}
  Workload $\mathbf{R}_{k^d}$ can be answered with 
  \begin{equation*}
    O(\theta ^2 \cdot \frac{d^3 \log^{3(d-1)}k}{\epsilon^2})
  \end{equation*}
  error per query under  $(\epsilon, G^\theta_{k^d})$-Blowfish privacy.
\end{corollary}
\begin{proof}
  This follows from Lemma~\ref{lem:subgraph} and Theorem~\ref{thm:range-dd}. For each pair of nodes $u$ and $v$ such that $(u,v)$ is an edge in $G^\theta_{k^d}$, $u$ and $v$ are connected by a path of at most $\theta$ in $G^1_{k^d}$.
\end{proof}

This strategy is a good one as long as $\theta$ is a small constant. As $\theta$ grows, according to our lower bound results the minimum error under $(\epsilon, G^\theta_{k^d})$-Blowfish privacy approaches the minimum error under $\epsilon$-bounded differential privacy. 

